In-situ measurements of the intrinsic emittance of photocathodes for high brightness electron beams

The beam parameters of complete prototype of the bERLinPro injector that consisted of a lead cathode in an 1.6 cell superconducting cavity were measured. The measurements are discussed in chapter 2 and indicate that the beam emittance is governed by a multitude of contributions from the cathode and the injector. Cathodes for practical use must have a high enough QE to deliver the required current at moderate illumination intensities and be able to sustain the operation for several days. Alkali antimonides are good candidates for this purpose, as discussed in chapter 3.2. The preparation of such cathodes with QEs of a few percent in the visible range has been performed routinely but the details of the growth and the influence of process parameters on the cathodes properties are not well understood yet. A theoretical treatment of photoemission is presented, and expressions for quantum effciency and initial emittance of photocathodes are reviewed in section 3.1. In order to study Potassium Caesium Antimonide (K2CsSb) cathodes and their fabrication a preparation and characterization system has been developed at HZB. In section 3.2 this experimental setup is explained, details of the alkali antimonide cathodes are discussed, and the preparation of a caesium antimonide cathode is presented. Finally, chapter 4 focuses on the physics and engineering design of spectrometer that will resolve the initial transverse momentum of the photoelectrons released from cathode samples, the momentatron. It is installed in the analysis chamber of the cathode preparation system and allows in-situ characterization of the samples.

==> abbreviations.tex <==
\chapter*{Abkürzungen}


\begin{tabular}{ll}
 Abkürzung & Erklürung    \\
 \hline
      z.B. & zum Beispiel \\
\end{tabular}



==> abstract.tex <==
%-englische-Zusammenfassung---------------------------------------

\selectlanguage{english}

\begin{abstract}
\setcounter{page}{2} % Nach Bedarf anpassen!
Here is the english abstract.


% hier werden die englische Schlagwörter aus Metadaten übernommen
\dckeywordsen				
\end{abstract}

%-deutsche Zusammenfassung----------------------------------------

\selectlanguage{ngerman}

\begin{abstract}
\setcounter{page}{3} % Nach Bedarf anpassen!
Hier kommt die deutsche Zusammenfassung.


% hier werden die deutsche Schlagwörter aus Metadaten übernommen
\dckeywordsde
\end{abstract}



==> cv.tex <==
\chapter*{Lebenslauf}

%

\begin{tabular}{ll}

Name: & \dcauthorname  \dcauthorsurname \\

10.1994--09.1995 & Studium an der Humboldt-Universität zu Berlin \\

 & in der Fachrichtung Biologie\\

10.1995--11.1996 & Wissenschaftliche Mitarbeiterin an \\

 & der Humboldt-Universität zu Berlin,\\

 & Lehrstuhl Prof. XY, \\

 & Institut für Biologie\\

\end{tabular}


==> dedication.tex <==
\chapter*{Widmung}
Hier folgt dann eine Widmung.

==> emittance_old.tex <==
\section{Emittance}

In order to obtain the normalized rms emittance

\begin{equation}
\varepsilon_n :=  \beta \gamma \sqrt{<x^2><x^{\prime2}>-<xx'>^2}
\end{equation}

it is assumed, that the emission occurs uniformly from a circular illuminated spot on the cathode surface with radius $r$, thus $<x^2> = r/2$. Furthermore, because the emittance is considered just outside the cathode surface, where electron flow is laminar, the correlation term can be neglected. $\beta$ and $\gamma$ are the relativistic factors that normalize the emittance with respect to the average kinetic energy.

%Consider a young electron, that just emerged from the cathode surface. It's transverse momentum was conserved during passage of the surface barrier (assuming no scattering occurred at the barrier). Thus, the normalized emittance is conserved \cite{Flottmann1997}. We can move the integration over the transverse momentum distribution from outside (cold, vast vacuum) to the inside of the cathode crystal, where electrons feel home. Here, they can be lured into treatment with well known results of solid state theory.

--- \textbf{Dowell} starts from electron distribution function $g$

\begin{equation}
<p_x^2> = \frac{\int dE \int d(\cos \Theta) \int d\varphi \, g(E,\Theta,\varphi) \, p_x^2}{\int dE \int d(\cos \Theta) \int d\varphi \, g(E,\Theta,\varphi)}
\end{equation}

Integration considers the momentum distribution inside of the cathode. The transverse momentum is conserved during emission through the surface barrier (assuming no scattering occurs at the barrier). Thus, the normalized emittance is conserved.

\begin{equation}
g_{photo} = (1-f_{FD}(E+\hbar \omega))f_{FD}(E)
\end{equation}
Fermi-Dirac distribution is well represented by a Heavyside step-function which determines the limits of the integration.
The $\Theta$ integration rages from zero to $\Theta_{max}$

\begin{equation}
<p_x^2> = \frac{\int\limits_{E_F+\Phi_{eff}-\hbar\omega}^{E_F} dE \int\limits_{\sqrt{\frac{E_F + \Phi_{eff}}{E+\hbar\omega}}}^{1} d(\cos \Theta) \int\limits_{0}^{2\pi} d\varphi \, (E+\hbar\omega) \, \sin^2\Theta \, \cos^2\varphi}{\int dE \int d(\cos \Theta) \int d\varphi}
\end{equation}

\begin{equation}
\varepsilon_{photo} = \sigma_x \sqrt{\frac{\hbar\omega - \Phi_{eff}}{3mc^2}}
\end{equation}


--- In this work, the ansatz proposed by \textbf{Jensen} \cite{Jensen2006, Jensen2007} is followed and slightly modified to the treatment of semiconductors instead of metals. The ansatz includes the three-step model of photoemission, makes use of step-functions as approximations for densities of states as well as emission probabilities. Scattering is neglected, this strong approximation is maintainable because electron-electron scattering is nearly absent in semiconductors and the cathodes will be operated at temperatures well below room temperature, so electron-phonon scattering will also have negligible effect. The existence of valence and conduction band is included implicitly by adapting the integration ranges. Explicit consideration of the band structure and density of states could be tackled in a numerical model, calculated band structures of K$_2$CsSb and KCs$_2$Sb have been published by Ettema et al. and Kalarasse et al. \cite{Ettema2002, Kalarasse2010}.

We follow Jensen to the point, that the $n$-th moment of the transverse momentum of the excited electrons inside the crystal is

\begin{equation}
M_n = \int k_x^n \, f(E(\vec{k})) \, k^2 sin \vartheta \dd \varphi \dd \vartheta \dd k
\end{equation}

The integration is transformed from the absolute value of the momentum to energy and, following Dowell's argument, we integrate over the augmented energy ($E+\hbar\omega$):

\begin{eqnarray}
\vec{k} &=& \sqrt{  \frac{2m(E+\hbar\omega)}{\hbar^2} } \\
\dd k   &=& \frac{1}{2} \sqrt{ \frac{2m}{\hbar^2} } (E+\hbar\omega)^{1/2} \dd E \\
M_n     &=& \frac{1}{2} (\frac{2m}{\hbar^2})^{3/2}\int (\frac{2m}{\hbar^2})^{n/2} (E+\hbar\omega)^{\frac{n+1}{2}} \, f(E(\vec{k})) \,  sin^{n+1} \vartheta cos^n \varphi \dd \varphi \dd \vartheta \dd E
\end{eqnarray}

Now restrict $\vartheta$ integration to escape cone, integrate energy over correct interval, see what comes out!

\textbf{see also derivations in appendix}



\begin{figure}[!hb]
\label{fig:semiconductor-bands}
\includegraphics[width=0.85\textwidth]{../img/e-bands-semicond.pdf}
\caption[Schematic band structure of a semiconductor and emission processes]{Schematic band structure of a semiconductor and emission processes (Fig. from \cite{Clendenin1998}).}
\end{figure}

\begin{figure}[!hb]
\label{fig:e-bands}
\includegraphics[width=\textwidth]{../img/e-bands-compare.pdf}
\caption[Schematic band structure of metals and semiconductors]{Schematic band structure of metals and semiconductors.}
\end{figure}

==> gun.tex <==
\chapter{Emittance Measurements of a Superconducting High Frequency Electron Gun}
%
%\footnote{test}
\label{chap:measuring-emittance}

\section{Measurement of the Emittance}

Two techniques to measure the emittance are discussed: both yield the aforementioned rms emittance, one by summing up second moments of the particle distribution, the other by fitting parameters that depend on the rms distribution. Statistical information about the beam is obtained by peak finding algorithms that are applied to the measured intensity distribution. \footnote{The work contained in this chapter was previously published in a status report.}

\subsection{Slit Based Technique}
\label{chap:slit}

The slit mask measurement allows to reconstruct the projected phase space distribution in one transverse direction at the location of the slit, as illustrated in figure \ref{fig:scheme-slit-mask}. The slit serves two purposes. For one, the slit selects a narrow band of the particle distribution, which allows to scan the beam's diameter and correlate transverse position and divergence. The width and mean value of the divergence of the beamlet are calculated from the transverse distance travelled in a drift path. Furthermore, if the beam dynamics upstream of the slit is space charge dominated, the aperture reduces the bunch charge so one may assume emittance dominated dynamics in the downstream beamlet. Space charge effects on the beamlet are neglected in this work, but do have an influence on the measured emittance at higher bunch charges \cite{Bazarov2008}.

\begin{figure}[ht]
\centering
\includegraphics[width=.75\textwidth]{scheme-slit-mask-measurement-abstract}
\caption{Schema of the measurement setup for a slit mask measurement.}
\label{fig:scheme-slit-mask}
\end{figure}

The emittance can be evaluated using equation \ref{eq:eps-definition} and the second moments as noted hereafter.
$y$ and $y'$ denote spatial positions of particles on a screen, $u_y$ and $u_y^\prime$ denote phase space coordinates for vertical position and divergence as indicated in figure \ref{fig:real-and-phase-space}:

\begin{equation}
\langle u_y^2 \rangle_{Beam} = \frac{\sum\limits_i^{Particles} y_{i}^2}{\sum\limits_i^{Particles} 1} = \frac{\sum\limits_j^{Beamlets} I_j \langle y^2 \rangle_{j}}{\sum\limits_j^{Beamlets} I_j}
\end{equation}

\begin{equation}
\langle u_y^{\prime 2} \rangle_{Beam} = \frac{\sum\limits_i^{Particles} y_i^{\prime 2}}{\sum\limits_i^{Particles} 1} =
 \frac{\sum\limits_j^{Beamlets} I_j  \langle y^{\prime 2} \rangle_j}{\sum\limits_j^{Beamlets} I_j} =
 \frac{\sum\limits_j^{Beamlets} I_j ( \mu_j^2 + \sigma_j^2 )}{\sum\limits_j^{Beamlets} I_j} 
\end{equation}

\begin{equation}
\langle u_y u_y^{\prime} \rangle_{Beam} = \frac{\sum\limits_j^{Beamlets} I_j \langle y\rangle_j \langle y^{\prime}\rangle_j}{\sum\limits_j^{Beamlets} I_j}
\end{equation}

here, $I_j$ is the measured intensity of the $j$-th beamlet on the screen, $\mu_j$ and $\sigma_j$ are center and standard deviation of an assumed normal distribution of the individual divergences $y^{\prime}_i$ in one beamlet.\\
Note, that in case of steering $y$ and $\mu_j$ need to be corrected for the collective divergence due to beam steering:

\begin{equation}
y^{\prime} = \frac{\tilde{y}^{\prime} - \alpha L}{l_{beamlet}}
\end{equation}

\begin{equation}
\mu_j = \langle y^{\prime} \rangle = \frac{\langle \tilde{y}^{\prime} \rangle - \alpha L}{l_{beamlet}}
\end{equation}

where $\alpha$ is the steering angle, $l_{beamlet}$ is the drift length of the beamlet between slit mask and screen and $L$ is the length between steerer and screen. $\tilde{y}^{\prime}$ denotes the measured position on a screen, that is shifted by the steerer angle.

\begin{figure}[ht]
\centering
\includegraphics[width=.75\textwidth]{real-and-phase-space-slit-mask-measurement}
\caption{Illustration of real and phase space distributions during a slit mask measurement.}
\label{fig:real-and-phase-space}
\end{figure}

%Cite :

%Multislit \cite{Anderson2002}

%EMSY, Pitz \cite{DissStaykov, DissAsova}

\clearpage
\pagebreak
\subsection{Solenoid Scanning}

Using the solenoid to scan the beam waist through a screen yields information about the initial beam size, divergence and their correlation.
Photoinjectors are equipped with an emittance compensating solenoid that is used for these measurements.
In a linear beam optics model, the beam radius at the screen depends quadratically on the solenoid's focal length \cite{myVolker2012},  as illustrated in figure \ref{fig:scheme-solenoid-scan}b:

\begin{figure}[ht]
\centering
\includegraphics[width=.75\textwidth]{scheme-solenoid-measurement-abstract}
\caption[Schema of the measurement setup for a solenoid scan]{Schema of the measurement setup for a solenoid scan (a) and illustration of the quadratic fit to obtain parameters for the emittance calculation (b).}
\label{fig:scheme-solenoid-scan}
\end{figure}

\begin{equation}
\langle r_{f,L}^2 \rangle = \langle ( r_i + r_f^\prime \cdot L)^2 \rangle
\end{equation}

\begin{equation}
r_f^\prime = r_i^\prime - \frac{r_i}{f}
\end{equation}

\begin{equation}
\langle r_{f,L}^2 \rangle = \frac{1}{f^2} \underbrace{(\langle r_i^2 \rangle L^2)}_a + \frac{1}{f} \underbrace{(-2L(L\langle r_i r_i^\prime \rangle + \langle r_i^2 \rangle))}_b + \underbrace{\langle r_i^{\prime 2} \rangle L^2 + 2L\langle r_i r_i^\prime \rangle + \langle r_i^2 \rangle}_c
\end{equation}

\begin{equation}
\varepsilon_{rms} = \frac{\sqrt{ac-\frac{b^2}{4}}}{L^2}
\end{equation}
where L is the distance between solenoid and screen, $r$ and $r'$ are the radial position and divergence of a particle at initial (before solenoid) and final (screen) positions, indicated by an i or f subscript, respectively.
The parameters $a, b$ and $c$ can be obtained from a quadratic fit of the beam size, plotted against the inverse focal lengths of the solenoid.

%%% kein Vorgriff auf Ergebnisse, ist dort schon ausfühlicher diskutiert!
%Strongly focusing the beam may introduce errors due to aberrations of the solenoid.
%Spherical aberrations depend on higher moments of the beam's trace space distribution and are negligible in this case due to the small beam diameter.
%The chromatic aberration depends linearly on the energy spread of the beam and may cause an overestimation of the emittance.
%Due to the rotation of the beam by the larmor angle $\Theta_L$, the astigmatism of the solenoid may lead to a vast overestimation of the beam's diameter and emittance when measuring in the laboratory frame, which is not rotated.

%\begin{figure}[ht]
%\centering
%\includegraphics[width=.75\textwidth]{results-0.2/sol-example}
%\caption{Illustration of the quadratic fit to the beam size.}
%\label{fig:quad-fit}
%\end{figure}

\subsection{Numerical Tracing of Particle Trajectories}

Numerical tracing of particle trajectories with ASTRA \cite{Astra} has been used to validate the analysis scripts used for the measured slit mask data. Further investigations regarding the influence of slit aperture and distances on measurement accuracy of the slit mask measurements are envisaged.
Particle tracking was also employed to obtain an estimate on the momentum spread of the beam, which was not possible to measure with the current setup but is required to estimate the chromatic aberration of the solenoid.

\section{Experimental Setup}
\label{chap:Setup}

An SRF injector is driven by a laser source that extracts photoelectrons from a cathode. The cathode is located in the back wall of an RF cavity where the electron bunches are accelerated by a strong electric field gradient, timed to match the correct phase of the RF wave.
The beam is fed into a diagnostics beam line, where fundamental beam parameters can be measured.

\begin{figure}[ht]
\centering
\includegraphics[width=.75\textwidth]{beamline}
\caption[HoBiCaT cryomodule and the diagnostic beamline]{Overview of the HoBiCaT cryomodule and the diagnostic beamline.}
\end{figure}

\subsection{Electron Gun}

The electron gun is the second prototype ("Gun 0.2") in a step-by-step approach towards the \berlinpro~injector.
It consists of a 1.6 cell superconducting niobium cavity that is located in the HoBiCaT cryostat, at an operational temperature of 1.8\,K, and a cathode plug inserted into the back wall of the cavity.
The cavity was fed with microwave power from an inductive output tube (IOT) or a solid state amplifier at 1.3\,GHz and was operated at field gradients up to 28\,MV/m, limited by field emission followed by slow quench. Stable operation was possible up to 27\,MV/m.
The cathode plug was made of niobium covered with a thin lead film. Lead has an approximately one order of magnitude higher quantum efficiency but is also superconducting below 7.2\,K.
Table \ref{tab:gun-parameters} lists typical operational parameters of the gun.

\begin{table}[!ht]
\centering
\setlength{\arrayrulewidth}{0.25pt}
\begin{tabular}{c c c}
\hline 

\textbf{Parameter} & \textbf{Value} & \textbf{Unit}    \\ \midrule

Average Current    & $<$ 1          & nA               \\ \midrule
Bunch Charge       & 0.187          & pC               \\ \midrule
QE                 & $10^{-5}$      &                  \\ \midrule
Beam Energy        & 1-2.5          & MeV              \\ \midrule
Laser Power        & $<$ 0.5        & mW               \\ \midrule
Laser wavelength   & 258            & nm               \\ \midrule
Pulse Length       & 2.5 \ldots 3   & ps fwhm, gaussian\\ \midrule
Rep rate           &  8             & kHz              \\ \midrule
$\mathrm{E_{max}}$ & \parbox{5cm}{\centering 10 - 12.5 w solid amp\\ 22 with IOT\\ 27 peak field} & MV/m  \\ 
\hline 
\end{tabular}
\caption[Operational Parameters of Gun 0.2]{Typical operational parameters of Gun 0.2 with a lead coated cathode. The pulse length refers to the emission time of the bunch. }
\label{tab:gun-parameters}
\end{table} 

\subsection{Diagnostic Beam Line}

Several screens were employed to image beam profiles and to aid beam positioning. 
The solenoid can be used to focus the beam on the front or back screens in the straight beam line,
where a solenoid scan yields emittance information as described in subsection \ref{chap:measuring-emittance}.
A superconducting solenoid with an effective magnetic length of 41.5\,mm and a field amplitude of $44.1\,\frac{\mathrm{mT}}{\mathrm{A}}$ \cite{myVolker2012} was located inside the cryomodule.
The distance between the cathode and the center of the solenoid was 439\,mm.
Three beam stops made of copper served as faraday cups for current measurements. They were located at the first screen station and at the two ends of the beamline.

The slit at the first screen station was used to select a narrow beamlet which was imaged on the back screen.
The slit mask was made of 1.5\,mm thick tungsten with an $100\,\mu$m aperture and located directly in front of the first screen and faraday cup. A thickness of 1.5\,mm gives a good compromise between efficient suppression of the background and sufficient transmission.

%A bending dipole and the screen in the dispersive subsection were used to measure the beam momentum.
In the dispersive subsection, after the beam has passed the dipole, it was possible to evaluate the momentum of the particles. Because the dipole could not be driven into saturation it was calibrated by cycling between +8\,A and -8\,A \cite{myMatveenko}. The beam momentum can be calculated as

\begin{equation}
pc = 0.88 \cdot \left( \frac{I_{Dipole}}{[A]} + 0.12 \right) [MeV].
\end{equation}



\subsection{Procedures}

Three individual measurements were conducted to characterize the phase space of one beam setting using the slit mask. First, the beam was imaged on the front screen without slit to calibrate the steerer angle and vertical offset. In a second sweep the front screen was used again, but with the slit to measure the beamlet intensity. Finally, the beamlets were allowed to drift towards the back screen in order to measure the divergence of each beamlet.
All measured values were taken from ten polls per beamlet on the back screen and five polls per beamlet on the front screen. Mean and standard deviation were recorded.
The phase space distributions were corrected for the steerer angle and summed up to obtain second moments and the emittance as described in \cite{Anderson2002}.

In order to conduct a solenoid scan, the current in the solenoid was varied over a specified range \cite{myVolker2012}.
Screen images were saved for a single poll per solenoid setting,
while beam positions and diameters were averaged over six polls. 
Beam parameters and the emittance are obtained from a quadratic fit of the beam width against the inverse focal length of the SC solenoid.

\section{Results}
\label{chap:results}

All measurements were conducted in November 2012 during the last run of the "Gun 0.2" setup. At that time, the cavity was operated with full RF power from the IOT only for test measurements and energy calibration. Due to a failure in the power supply of the IOT only up to 12.5\,MV/m were available for the subsequent beam measurements using a solid state amplifier.

\subsection{Slit Mask Measurements}

The vertical phase space was characterized at different laser spot sizes with a constant cavity gradient of 10\,MV/m at an emission phase of approximately 15\,deg using the slit mask as described in subsection \ref{chap:slit}. An aperture in the laser beam line was used to manipulate the spot size, however, other laser settings remained constant so the bunch charges were not equalized among the measurements (but all below the space charge regime). At a spot size of 0.46\,mm\,rms three solenoid settings were studied. The resulting emittance values are displayed in figure \ref{fig:slit-mask-results}.

\begin{figure}[ht]
\centering
\includegraphics[width=.75\textwidth]{results-0.2/steerer-eps-err}
\caption[Results of emittance measurements using the slit mask technique]{Results of emittance measurements using the slit mask technique. Bunch charges are not equal.}
\label{fig:slit-mask-results}
\end{figure}

A linear dependency of the normalized emittance with respect to the rms laser spot size can be recognized, despite the scattering of the data. The corresponding phase spaces are displayed in figure \ref{fig:phase-spaces-laser}, where at large spot sizes a structured phase space was obtained. This hints at structured emission from hot spots on the cathode surface which may be covered with protrusions and droplets.

Uncertainties due to temporal deviations and other statistical errors are estimated to amount to less than 5\,\%. The finite thickness of the YAG screen together with a 45\,deg viewing angle may introduce an overestimation of the measured beam size of up to 30\,$\mu$m \cite{myBardayIBIC2012}. From a numerical estimate this will introduce a systematic error of about +3\,\% in the emittance. Space charge effects are negligible at the observed bunch charges below 1\,pC. Only these effects are taken into account by the error bars in figure \ref{fig:slit-mask-results}.

The accuracy of the evaluated emittance is largely defined by the dynamic range of the entire measurement, which differs between measurements because beamlets at the tail of the distribution might move off the screen due to geometrical constraints.
The range differs between 2.5 and 6.4\,dB, which implies that differences as large as
20\,\% in the number of considered particles occur.
For reference, a simulated charge cut curve in figure \ref{fig:charge-cut} shows the dependence of the emittance on the amount of particles imaged.

\begin{figure}[ht]
\vspace{-0.1cm}
\centering
\includegraphics[width=.45\textwidth]{results-0.2/core-eps-simulated}
\caption{Simulated charge cut curve of a round beam from the photoinjector.}
\label{fig:charge-cut}
\end{figure}


\begin{figure}[ht]
\centering
\mbox{\includegraphics[width=.5\textwidth]{phase-spaces/laser/PhaseSpace-920mA-spot3-FWHM}
\includegraphics[width=.5\textwidth]{phase-spaces/laser/PhaseSpace-920mA-1127-FWHM}}
\mbox{\includegraphics[width=.5\textwidth]{phase-spaces/laser/PhaseSpace-920mA-FWHM}
\includegraphics[width=.5\textwidth]{phase-spaces/laser/PhaseSpace-920mA-spot2-FWHM}}
\caption[Reconstructions of vertical phase spaces with different laser spot sizes]{Reconstructions of vertical phase spaces, laser spot size increases in reading direction and is indicated in the figures.}
\label{fig:phase-spaces-laser}
\end{figure}


\clearpage
Three measurements with identical beam settings but increasing solenoid current were performed. The phase spaces are printed in figure \ref{fig:phase-spaces-sol}. The correlation between the vertical position and divergence is clearly increasing with the solenoid current as the focal point moves closer to the solenoid.
\begin{figure}[ht]
\centering
\mbox{\includegraphics[width=.5\textwidth]{phase-spaces/PhaseSpace-820mA-FWHM}
\includegraphics[width=.5\textwidth]{phase-spaces/PhaseSpace-920mA-FWHM}}
\includegraphics[width=.5\textwidth]{phase-spaces/PhaseSpace-1020mA-FWHM}
\caption[Reconstructions of vertical phase spaces at different solenoid currents]{Reconstructions of vertical phase spaces at increasing solenoid currents, as indicated in the figures.}
\label{fig:phase-spaces-sol}
\end{figure}

\subsection{Solenoid Scans}

Emittance measurements with different laser spot sizes were also carried out using the solenoid scan, see figure \ref{fig:sol-scan-laser}. The data was taken with a field amplitude of 10\,MV/m at launch phases of 15 and 25\,deg, which corresponds to beam energies of 0.94 and 0.90\,MeV, respectively. The beam was imaged on the front screen, at a distance of 1.121\,m to the center of the solenoid coil. As was observed with the slit mask measurements, the data shows a linear dependency, however, the values are slightly larger in this case.

%%
% figure emittance vs laser
%%
\begin{figure}[!ht]
\centering
\includegraphics[width=.75\textwidth]{results-0.2/sol-scans-laser-xy}
\caption[Emittance measurements using the solenoid scan technique at different laser diameters]{Emittance measurements using the solenoid scan technique at different laser diameters. Bunch charges are not equal. The lower values are from measurements at 15\,deg launch phase, the higher ones at 25\,deg. Horizontal and vertical fits are for the 15\,deg measurement only.}
\label{fig:sol-scan-laser}
\end{figure}

Additionally, emittance measurements for different emission phases were conducted at a gradient of 12.5\,MV/m.
The resulting emittances are displayed in figure \ref{fig:PhaseScan-emittances}.
For reference, the corresponding average currents and beam energies can be found in figure \ref{fig:PhaseScan-current-energies}.
The emittance rises linearly with the launch phase up to 30\,deg and seems to flatten between 30 and 40\,deg.

Values measured using the front screen are clearly larger than the ones measured on the back screen.
Starting from 5\,\% at low launch phases the difference increases also linearly with the phase to up to 20\,\% at phases of 30 and 40\,deg.
Higher emittance values on the front screen, where the beam has to be focused stronger, suggest that strong focussing introduces aberrations that lead to an increase of the emittance.
The effect of chromatic and spherical aberrations of the solenoid was investigated with several simulations in \cite{myVolker2012}.
For similar beam parameters and the same solenoid it was shown that the spherical aberration coefficient $C_s$ increases from about 630~m$^{-3}$ to about 960~m$^{-3}$ when moving the focus from the back to the front screen.
The emittance increase due to spherical aberrations depends on higher-order moments of the particle distribution \cite{myVolker2012}:
\begin{equation}
\varepsilon^2 = \varepsilon^2_{(lin)} + 2 \, C_s\left(\langle r^3_i r_i^\prime \rangle \langle r_i^2 \rangle - 3 \langle r_i r_i^\prime \rangle\langle r_i^2 \rangle^2 \right) + 6 \, C_s \, \langle r_i^2 \rangle^4
\end{equation}
which are not known, however a rough estimate with values from simulations and the slit mask measurements yields an emittance increase that is several orders of magnitude lower than the measured difference.

The chromatic aberration follows \cite{Dowell}
\begin{equation}
\varepsilon_{n,chrom} = \sigma^2_{x,sol} \, \frac{\sigma_p}{mc} \, K |\sin KL + KL \cos KL|
\end{equation}
where $\sigma_{x,sol}$ is the rms beam width at the solenoid, $\sigma_p$ is the rms momentum spread, $K=\frac{eB_0}{2p}$ and $L$ is the solenoid's effective length. Because no vertical slit was installed in front of the dipole, a precise measurement of the momentum spread was not possible. The influence of the chromatic aberration was estimated using beam size and momentum spread values from Astra simulations. As can be seen in figure \ref{fig:chromaticity}, the influence is much stronger when focusing the beam on the front screen. Overall, the chromatic aberration may be responsible for the increase of the measured emittance with the launch phase as it also increases nearly linearly below 30\,deg and flattens above 30\,deg. Additionally, it explains the discrepancy between the measurements on the front and back screen, because focusing on the front screen introduces higher aberrations due to the stronger solenoid field.

A third source of uncertainty is caused by the astigmatism of the solenoid. It causes two separated foci for the two transverse directions. When the beam is focused in $x$ direction, it may still have twice its minimal size in $y$ direction and vice versa. Because the beam is rotated by the larmor angle $\Theta_L$ with respect to the lab frame, this may result in a vast overestimation of the beam diameter on the screen and, subsequently, of the reported emittance. This effect is especially prominent in the measurements on the front screen. It is assumed that the difference between the horizontal and vertical emittance in the measurements on the front screen is due to the astigmatism. The lower uncertainty level was estimated to
\begin{equation}
\Delta \varepsilon = C \, \sigma_y\bigg|_{\sigma_x = min} \, \sin(\Theta_L)
\end{equation}
where $\sigma_y$ is the beam diameter in $y$ direction at the location of the beam waist in $x$ direction. C is a constant and was set to 0.25 for the present results. It is somewhat arbitrary because the influence of the larmor rotation on the projected intensity is not known for the specific distribution.
Chromatic aberration and astigmatism effects are accounted for in the error bars of figure \ref{fig:PhaseScan-emittances}.

%%
% figure emittance vs phase
%%
\begin{figure}[ht]
\centering
\includegraphics[width=.75\textwidth]{results-0.2/PhaseScan-emittances-error}
\caption[Emittance measurements for different emission phases]{Emittance measurements for different emission phases on the front and back screen. Error bars account for chromatic aberration and astigmatism.}
\label{fig:PhaseScan-emittances}
\end{figure}

%%
% figure current vs phase
%%
\begin{figure}[ht]
\centering
\includegraphics[width=.75\textwidth]{results-0.2/PhaseScan-current-energies}
\caption{Phase scan of the beam current and energy.}
\label{fig:PhaseScan-current-energies}
\end{figure}

%%
% figure chromatic aberration of the solenoid
%%
\begin{figure}[ht]
\centering
\includegraphics[width=.75\textwidth]{results-0.2/chromaticity}
\caption[Influence of the chromatic aberration of the solenoid on the beam emittance]{Influence of the chromatic aberration of the solenoid on the beam emittance for a beam at 12.5\,MV/m accelerating gradient. Front and back refers to solenoid settings where the beam is focused on the front and back screen, respectively.}
\label{fig:chromaticity}
\end{figure}

==> hyphenations.tex <==
% Tragen Sie Ihre eigenen Trennregel ein:
\hyphenation{Bei-spiel, Ö-ko-lo-gie}

==> introduction.tex <==
\chapter{Introduction}

Electron sources for applications in accelerator technology cover a broad spectrum of applications.
They are employed in large scale facilities where the electron beam is essential to operation, like synchrotron light sources, Compton X-ray sources or electron colliders.
Another application is the generation of electron beams which are used to support the operation of a different facility, for example for electron cooling of ion beams.
Over the last decades, development on several types of sources improved the beam parameters and lead to specialized sources, tailored to the specific demand of the application.
Generally, a common goal for all types of sources is to provide beams with high brightness, high average current and, where applicable, in continuous-wave operation.

Synchrotron light sources commonly use thermionic DC guns with buncher cavities (BESSY II and NSLS II, for example) or a thermionic cathode inside a normal conducting radio frequency cavity (APS and SSRL) as sources for the low energy bunched beam which is subsequently accelerated to the energy of the storage ring.

High gradient electrostatic (DC) photoinjectors are used mainly for application of GaAs photocathodes. These photocathodes provide a high quantum efficiency (QE) and spin polarized electron beams but have very stringent vacuum requirements that cannot be met in a normal conducting RF gun.

The development of superconducting RF cavities with low losses allows to operate SRF photoinjectors at high gradients of several 10\,MV/m in continuous wave (cw) mode.
Additionally, these cavities provide vacuum conditions suitable for application of GaAs or alkali antimonide photocathodes. SRF photoinjectors feature a photocathode on the back wall of the first half cell of the cavity structure.
A drive laser is coupled in and excites a short electron bunch that is released in the accelerating part of the RF period.
The concept was first developed at Los Alamos \cite{Fraser1985} and and is now actively developed in several projects, for example at Helmholtz-Zentrum Berlin (HZB) \cite{Neumann2012}, Helmholtz-Zentrum Dresden Rossendorf \cite{Arnold2007} and Brookhaven National Lab \cite{Belomestnykh2012}.
The advantages of an SRF photoinjector
%when compared to a normal conducting or photoinjector are the operation at high launch gradients in cw mode with low RF losses and vacuum conditions that allow the use of sensitive semiconducting cathodes. These 
come at the expense of a complex cryogenic infrastructure and its operational costs. 


At Helmholtz-Zentrum Berlin, a high-brightness electron source which will use the SRF photoinjector concept is under development for the prospected energy recovery linac bERLinPro \cite{bERLinPro-CDR}. Energy recovery linacs (ERLs) will deliver high brightness beams where the fundamental limit is set by the beam source instead of equilibrium conditions as in storage rings. At the same time, they allow cw operation at high currents where management (dumping) of the spent high energy beam and operational cost forbid such modes in conventional linacs. Thus, ERLs hold the promise to combine the advantages of linear accelerators and storage rings.
bERLinPro is intended as 
%a technology incubator and
a demonstration facility for high current, cw operation of an ERL. It will accelerate a 100\,mA electron beam to 50\,MeV with a 1.3\,GHz repetition rate.

The normalized brightness $B_n$ of a beam is an important figure of merit to characterise the beam of an accelerator. In a light source, the brightness of the photon beam depends on the peak brightness of the electron beam. For electron beams, brightness is defined as the beam current $I$ divided by its normalized trace space volume \cite{Reiser2008}:

\begin{equation}
B = \frac{2}{\pi^2} \frac{I}{\varepsilon_{x,n} \varepsilon_{y,n}} \, ,
\end{equation}

where $\varepsilon_n$ are the normalized emittances. Thus, the goals for the source are to provide a beam with low emittance, high peak current in short bunches and low energy spread. Specifically, for bERLinPro, the design beam parameters are 77\,pC bunch charge with an emittance below 0.5\,mm\,mrad in the injector and below 1.0\,mm\,mrad in the recirculator at an rms bunch length of 2\,ps.

The beam parameters of a lead cathode in an 1.6 cell superconducting cavity were measured in a test setup of the bERLinPro injector. The measurements are discussed in chapter \ref{chap:measuring-emittance} and indicate that the beam emittance is governed by two effects. A large fraction is contributed by field errors of the solenoid. The second influence is due to the surface quality and initial emittance of the photocathode which require further investigation and improvement. 
%
Photocathodes for practical use must have a high enough QE to deliver the required current at moderate illumination intensities and be able to sustain the operation for several days. Alkali antimonides are good candidates for this purpose, as discussed in chapter \ref{sec:alkali-antimonides}. The preparation of such cathodes with QEs of a few percent in the visible range has been performed routinely \cite{Cultrera2013,mySmedley2009} but the details of the growth and the influence of process parameters on the cathode's properties are not well understood yet.
A theoretical treatment of photoemission is presented, and expressions for quantum efficiency and initial emittance of photocathodes are reviewed in section \ref{sec:theory}.
In order to study Potassium Caesium Antimonide (\PCA) cathodes and their fabrication a preparation and characterization system has been developed at HZB.
In section \ref{sec:alkali-antimonides} this experimental setup is explained, details of the alkali antimonide cathodes are discussed, and the preparation of a caesium antimonide cathode is presented.
%Finally, the physics and engineering design of the spectrometer are covered in chapter \ref{chap:momentatron}.
Finally, chapter \ref{chap:momentatron} focuses on the physics and engineering design of spectrometer that will resolve the initial transverse momentum of the photoelectrons released from cathode samples, the momentatron. It is installed in the analysis chamber of the cathode preparation system and allows \textit{in-situ} characterization of the samples. 



%Light, in its common definition as the visible part of the electromagnetic spectrum, has been a vital source of information about our environment since the very first organisms developed the ability to sense light and paved the route to the evolution of the complex human visual system we depend on so heavily today : Most people use their vision to collect information about objects and events in their vicinity, thus, in a very personal, subjective way, but also very essential to everyday life.

%In a similar manner, researchers use light with well defined properties to shine on samples of matter and specialized detectors to record -- or "see" to stay with the comparison -- a manifold of processes that take place in the sample and reveal properties of the material.
%The light for this use may span a broader spectrum than the common definition and range from the far infrared to hard X-ray radiation. A large part of this spectrum can be covered by light sources that emit synchrotron radiation from highly energetic electron beams.

%In order to meet the demands of next-generation light sources, the electron source must fulfil tight beam parameters with respect to the longitudinal and transverse energy distribution and the temporal and transverse spatial distribution of the emitted electrons. To put it shortly, the 6-dimensional phase space volume populated by each bunch in a pulsed beam must be very small. At the same time, the beam intensity at the user stations is supposed to be as high as possible, so the small phase space volume of the bunch needs to be densely packed.

